Quantum and classical aspects of scalar and vector fields around black holes

This thesis presents recent studies on test scalar and vector fields around black holes. It is separated in two parts according to the asymptotic properties of the spacetime under study. In the first part, we investigate scalar and Proca fields on an asymptotically flat background. For the Proca field, we obtain a complete set of equations of motion in higher dimensional spherically symmetric backgrounds. These equations are solved numerically, both to compute Hawking radiation spectra and quasi-bound states. In the former case, we carry out a precise study of the longitudinal degrees of freedom induced by the field mass. This can be used to improve the model in the black hole event generators currently used at the Large Hadron Collider. Regarding quasi-bound states, we find arbitrarily long lived modes for a charged Proca field, as well as for a charged scalar field, in a Reissner-Nordstr\"om black hole. The second part of this thesis presents research on superradiant instabilities of scalar and Maxwell fields on an asymptotically anti-de Sitter background. For the scalar case, we introduce a charge coupling between the field and the background, and show that superradiant instabilities do exist for all $\ell$ modes, in higher dimensions. For the Maxwell case, we first propose a general prescription to impose boundary conditions on the Kerr-anti-de Sitter spacetime, and obtain two Robin boundary conditions. Then these two conditions are implemented to study superradiant unstable modes and vector clouds. In particular, we find that the new branch of quasinormal modes may be unstable in a larger parameter space. Furthermore, the existence of vector clouds indicates that one may find a vector hairy black hole solution for the Einstein-Maxwell-anti-de Sitter system at the nonlinear level, which implies that, in such system, the Kerr-Newman-anti-de Sitter black hole is not a unique solution.

==> abseng.tex <==
%% LaTeX2e file `abseng.tex'
%% generated by the `filecontents' environment
%% from source `tese' on 2015/12/09.
%%
\begin{longtable}{lX}
%\begin{tabularx}{\textwidth}{lX}
%
{\bf Keywords:} & black holes, Proca fields, Hawking radiation, TeV gravity, scalar fields, Maxwell fields, AdS, quasinormal modes, superradiance.\\
%
{\bf Abstract:} & This thesis presents recent studies on test scalar and vector fields around black holes in the classical theory of General Relativity. It is separated in two parts according to the asymptotic properties of the spacetime under study. In the first part, we investigate scalar and Proca fields on an asymptotically flat background. For the Proca field, using the Kodama-Ishibashi formalism, we are able to obtain a complete set of equations of motion in higher dimensional spherical symmetric backgrounds. These equations are solved numerically, both to compute Hawking radiation spectra and quasi-bound states. In the former case, for the first time, we carry out a precise study of the longitudinal degrees of freedom induced by the mass of the field. This can be used to improve the modeling of evaporation of black holes coupled to massive vector fields, and black hole event generators currently used at the LHC to probe TeV gravity models with extra dimensions. Regarding quasi-bound states, we find arbitrarily long lived modes for a charged Proca field in a Reissner-Nordstr\"om black hole. As a comparison, we also find such long lived modes for a charged scalar field. The second part of this thesis presents research on superradiant instabilities of scalar and Maxwell fields in an asymptotically anti-de Sitter (AdS) background. For the scalar case, we introduce charge coupling between the field and the background, and prove that superradiant instabilities do exist for all $\ell$ modes in higher dimensions. This result corrects a statement in the literature that such instabilities only appear in even dimensions. For the Maxwell case, we first propose a general prescription to impose boundary conditions on the Kerr-AdS spacetime, and obtain two Robin boundary conditions which give two different quasinormal modes even in a simpler Schwarzschild-AdS black holes. Then these two boundary conditions are implemented to study superradiant unstable modes and vector clouds. In particular, we find that the new branch of quasinormal modes may be more unstable. Furthermore, the existence of vector clouds indicate that one may find a vector  hairy black hole solution for the Einstein-Maxwell-AdS system in the nonlinear level, which imply that in such system Kerr-Newman-AdS black hole is not a unique solution.
%
%\end{tabularx}
\end{longtable}


==> analytics.tex <==
\chapter{Angular dependence of the news function}
\label{ch:analytics}

\epigraph{\emph{Sym\'etrie.} En ce qu'on voit d'une vue; fond\'ee sur ce qu'il n'y a pas de raison de faire autrement.}{Blaise Pascal\\ \emph{Pens\'ees}}

In the previous chapter we showed that the radiation signal seen by an infinitely far away observer, which when squared and integrated gives the energy radiated, is encoded in a sole function of retarded time $\tau$ and angular coordinate $\theta$. Furthermore, this so called news function depends exclusively on the transverse metric components $h_{ij}$, whose formal solution was given in integral form in Chapter~\ref{ch:dynamics}.

In this chapter we shall simplify that solution and study the angular dependence of the news function. We start in Section~\ref{CL} by showing that the metric possesses a conformal symmetry at each order in perturbation theory which, at null infinity, implies a factorisation of the angular dependence of the news function at each order. By actually computing that angular factor, we shall write the inelasticity's angular distribution as a power series in $\sin^2\theta$. In particular, we show that a consistent truncation of this angular series at $O(n)$ requires knowledge of the metric perturbations up to $O(n+1)$. This clarifies the meaning of perturbation theory in this problem: it allows for an angular expansion of the news function off the collision axis. In Section~\ref{asymp_waveforms} we simplify the integral solution and verify, explicitly, that it becomes effectively one-dimensional.

%%%%%%%%%%%%%%
\section{A hidden symmetry}
\label{CL}
%%%%%%%%%%%%%%
D'Eath and Payne observed, in $D=4$, that if one starts with a shock wave and performs a boost followed by an appropriate scaling of all coordinates, the end result is just an overall conformal factor \cite{D'Eath:1992hd}. This is easily understood in physical terms: since the only scale of the problem is the energy of the shock wave, the effect of the boost can be undone by rescaling the coordinates. In what follows we shall generalise this to $D\geq4$.

Recall the metric of one Aichelburg-Sexl shock wave in Rosen coordinates,
\begin{equation}
ds^2 = -d\bar{u} d\bar{v} + \left(1+\dfrac{\kappa \bar{u} \theta(\bar{u})}{2}\Phi''\right)^2d\bar{\rho}^{2} + \bar{\rho}^2\left(1+ \frac{\kappa \bar{u} \, \theta(\bar{u})}{2 \bar \rho}\Phi'\right)^2 d\bar{\Omega}^2_{D-3} \ .
\end{equation}
Now let $L$ be the Lorentz transformation
\begin{equation}
(\bar{u},\bar{v},\bar{x}^i)\xrightarrow{L}(e^{-\beta}\bar{u},e^\beta\bar{v},\bar{x}^i)\,,
\end{equation}
and $C$ the conformal scaling
\begin{equation}
(\bar{u},\bar{v},\bar{x}^i)\xrightarrow{C}e^{-\frac{1}{D-3}\beta}(\bar{u},\bar{v},\bar{x}^i)\,.
\end{equation}
Then, under the combined action of $CL$,
\begin{eqnarray}
(\bar{u},\bar{v},\bar{x}^i)&\xrightarrow{CL}&(e^{-\frac{D-2}{D-3}\beta}\bar{u},e^{\frac{D-4}{D-3}\beta}\bar{v},e^{-\frac{1}{D-3}\beta}\bar{x}^i)\,,\\
g_{\mu\nu}(\bar X)&\xrightarrow{CL}&e^{\frac{2}{D-3}\beta}g_{\mu\nu}(\bar X')\; ,
\end{eqnarray}
where $\bar X$ and $\bar X'$ denote the coordinates before and after the transformation respectively, i.e. $\bar X\xrightarrow{CL}\bar X'$. The metric simply scales by an overall factor.

Since this is a one parameter symmetry, one can find coordinates on $(D-1)$-dimensional sheets which are invariant under the transformation, and a normal coordinate parameterising inequivalent sheets. A suitable set of invariant coordinates on such sheets is $\left\{p,q,\phi^a\right\}$, with
\begin{equation}
p\equiv \bar{v}\bar{\rho}^{D-4}\,,\qquad q\equiv \bar{u}\bar{\rho}^{-(D-2)}\,, 
\end{equation}
and $\phi^a$ the angles on the transverse plane. The normal coordinate along the orbits of the symmetry is simply $\bar{\rho}$ which transforms as
\begin{equation}
\bar{\rho}\rightarrow\bar{\rho}'=e^{-\frac{1}{D-3}\beta}\bar{\rho}\,.
\end{equation} 

Now consider the superposition of two shocks. In the boosted frame with Rosen coordinates, the action of $CL$ is
\begin{equation}
g_{\mu\nu}(\nu,\lambda;\bar X)\xrightarrow{CL}e^{\frac{2}{D-3}\beta}g_{\mu\nu}(\nu,e^{-2\beta}\lambda;\bar X')\,.
\end{equation}
Thus the perturbative expansion remains the same except for $\lambda\rightarrow e^{-2\beta}\lambda$. In the centre-of-mass frame with Brinkmann coordinates, Eq.~\eqref{metric_series} becomes
\begin{eqnarray}\label{eq:CLonMetric}
g_{\mu\nu}(X) \xrightarrow{CL}g_{\mu\nu}(X')=e^{\frac{2}{D-3}\beta}\left[\eta_{ \mu \nu}+\sum_{k=1}^\infty e^{-2k\beta}  h_{\mu\nu}^{(k)}(X')\right]\,.
\end{eqnarray}
Quite remarkably, in the future of the collision the metric possesses a conformal symmetry at each order in perturbation theory.

Note that the metric functions $h_{\mu\nu}^{(k)}$ in Eq.~\eqref{eq:CLonMetric} are the same before and after the transformation, the only change being the coordinates they are evaluated on. On the other hand, for a generic coordinate transformation, the metric transforms as a rank-2 tensor,
\begin{equation}
g_{\mu \nu}(X)=\frac{\partial x^{\mu'}}{\partial x^\mu}\frac{\partial x^{\nu'}}{\partial x^\nu}g_{\mu' \nu'}(X')\,.
\end{equation}
Together with Eq.~\eqref{eq:CLonMetric} this implies that
\begin{equation}\label{CL_transf}
h_{\mu\nu}^{(k)}(X')=e^{(2k+N_u-N_v)\beta}h_{\mu\nu}^{(k)}(X)\,,
\end{equation}
where $N_u$ and $N_v$ are the number of $u$-indices and $v$-indices. Thus a given metric function evaluated on the transformed coordinates is the same function evaluated on the initial coordinates multiplied by an appropriate factor.

In these coordinates, the invariants $p,q$ read
\begin{equation}
p=(v-\Phi(\rho))\rho^{D-4}\,,\qquad q=u\rho^{-(D-2)}\,,\label{def_pq}
\end{equation}
while $\rho$ transforms as
\begin{equation}
\rho\rightarrow \rho'=e^{-\frac{1}{D-3}\beta}\rho\,.
\end{equation}

%%%%%%%%%%%%%%%%%%%%%
\subsection{Reduction to two dimensions}
%%%%%%%%%%%%%%%%%%%%%

Since $\rho$ is the only coordinate that transforms under the action of $CL$, Eq.~\eqref{CL_transf} implies a separation of variables in the form
\begin{equation}\label{eq:separation_rho}
h_{\mu\nu}^{(k)}(p,q,\rho,\phi^a)=\rho^{-(D-3)(2k+N_u-N_v)}f^{(k)}_{\mu\nu}(p,q,\phi^a)\,.
\end{equation}
Since the angles $\phi^a$ are ignorable, the problem becomes two dimensional at each order in perturbation theory. Let us see how.

In Section~\ref{reduction_3D} we defined scalar functions of $(u,v,\rho)$ by factoring out the trivial dependence of each metric component on $\phi^a$, Eqs.~\eqref{gen_perts}, and similarly for the sources $T^{(k-1)}_{\mu\nu}$. Then Eq.~\eqref{eq:separation_rho} implies that, for each of those functions generically denoted by $F(u,v,\rho)$ as before,
\begin{equation}
F^{(k)}(u,v,\rho)= \dfrac{f^{(k)}(p,q)}{\rho^{(D-3)(2k+N_u-N_v)}}\,.\label{f_pq}
\end{equation}
For its respective source as defined in Eq.~\eqref{def_S}, since the d'Alembertian operator scales as $\rho^{-2}$ under $CL$,
\begin{equation}
S^{(k)}(u,v,\rho)=\dfrac{s^{(k)}(p,q)}{\rho^{(D-3)(2k+N_u-N_v)+2}}\,.\label{def_s}
\end{equation}

Thus our problem is effectively two-dimensional in $(p,q)$ coordinates: at each order, $f^{(k)}(p,q)$ is the solution of a differential equation (inherited from the wave equation) with a source $s^{(k)}(p,q)$ and subject to initial conditions on $q=0$. This is an enormous computational advantage. In Section~\ref{app:Green2D} of Appendix~\ref{app:Green} we obtain the differential equation obeyed by $f^{(k)}(p,q)$ and the reduced Green's function $G^k_m(p,q;p',q')$. However, there is another consequence of this symmetry which only becomes manifest when one goes to null infinity.

%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The $CL$ symmetry at null infinity}
%%%%%%%%%%%%%%%%%%%%%%%%
In terms of $(r,\tau,\theta)$ the new coordinates $p$ and $q$ read
\begin{eqnarray}
p&=&(\tau+r(1+\cos\theta)-\Phi(r\sin\theta))(r\sin\theta)^{D-4}\,,\\
q&=&(\tau+r(1-\cos\theta))(r\sin\theta)^{-(D-2)}\,.
\end{eqnarray}
One can see they are not well-defined in the limit $r\rightarrow\infty$ since
\begin{equation}
p\rightarrow\infty\,,\qquad q\rightarrow0\,.
\end{equation}

However, it is reasonable to expect that the finite, non-trivial dependence of the news function in $(\tau,\theta)$ should be given in terms of combinations of $p,q$ that remain finite and non-trivial at null infinity. An appropriate choice is
\begin{equation}
\hat{p}\equiv
\left\{
\begin{array}{ll}
 \frac{pq-1}{q}+2\log q\ , &  D=4\  \vspace{2mm}\\
\displaystyle{ \frac{pq-1}{q^{\frac{1}{D-3}}}}\ , & D>4\ \label{tau_transform}\,
\end{array} \right. \ ,
\qquad \hat{q}\equiv q^{\frac{1}{D-3}}\,.
\end{equation}

This coordinate transformation, $(p,q)\rightarrow(\hat{p},\hat{q})$, has a constant non-vanishing determinant,
\begin{equation}
\det \left[\frac{\partial (p,q)}{\partial(\hat{p},\hat{q})}\right]=D-3\,,
\end{equation}
hence is well-defined everywhere.

When $r\rightarrow\infty$,
\begin{eqnarray}
\hat{p}&\rightarrow&2\bar{\tau}(\tau,\theta)+O\left(r^{-1}\right)\,,\\
\hat{q}&\rightarrow&(1-\cos\theta)^{\frac{1}{D-3}}(\sin\theta)^{-\frac{D-2}{D-3}}\times r^{-1}+O\left(r^{-2}\right)\,,
\end{eqnarray}
where we have defined a new time coordinate
\begin{eqnarray}
\bar{\tau}(\tau,\theta)=\left\{
\begin{array}{ll}
 \tau\times(1-\cos\theta)^{-1}+\log\left(\frac{1-\cos\theta}{\sin\theta}\right)\ , &  D=4\  \vspace{2mm}\\
\displaystyle{ \tau\times(1-\cos\theta)^{-\frac{1}{D-3}}(\sin\theta)^{-\frac{D-4}{D-3}}}\ , & D>4\ \label{tau_transform}\,
\end{array} \right. \ .
\end{eqnarray}

Recall that we had already factored out the $\rho$ dependence in Eq.~\eqref{f_pq}, leaving only a function of $(p,q)$ to compute. But since $\bar\tau$ is the only surviving quantity in the asymptotic limit, we expect the news function to become effectively one-dimensional at null infinity: besides the trivial dependence on $\theta$ coming from the known powers of $r$ and $\rho$ (remember that $\rho=r\sin\theta$), it must be a function of $\bar\tau(\tau,\theta)$ only.

From Eqs.~\eqref{news2} and \eqref{f_pq},
\begin{equation}
\dot{\mathcal{E}}^{(k)}(\tau,\theta)=(\sin\theta)^{\frac{D-4}{2}-2k(D-3)}\times\lim_{r\rightarrow\infty}\frac{d}{d\tau}\left[r^{\frac{D-2}{2}-2k(D-3)}\hat{f}^{(k)}(\hat{p},\hat{q})\right]\,,
\end{equation}
where $\hat{f}^{(k)}$ contains the relevant contribution from $E^{(k)}$ and $H^{(k)}$, as a function of $(\hat{p},\hat{q})$. 

If the quantity inside brackets is to remain finite at null infinity, then necessarily
\begin{equation}
\hat{f}^{(k)}(\hat{p},\hat{q})\simeq\alpha^{(k)}(\hat{p})\hat{q}^{\frac{D-2}{2}-2k(D-3)}+\dots\,,
\end{equation}
where $\dots$ denotes higher powers of $\hat{q}$ and $\alpha^{(k)}(\hat{p})$ some unknown function of $\hat{p}$. 

Thus, after taking the limit $r\rightarrow\infty$,
\begin{equation}
\dot{\mathcal{E}}^{(k)}(\tau,\theta)=\frac{1}{1-\cos\theta}\left(\frac{1+\cos\theta}{1-\cos\theta}\right)^{k-1+\frac{1}{4}\frac{D-4}{D-3}}\frac{d\bar\tau}{d\tau}(\theta)\times\frac{d}{d\bar\tau}\alpha^{(k)}(2\bar\tau)\,.
\end{equation}

Using Eq.~\eqref{tau_transform}, and evaluating this expression at $\theta=\tfrac{\pi}{2}$ noting that $\bar\tau\left(\tau,\tfrac{\pi}{2}\right)=\tau$, we conclude that
\begin{equation}
\dot{\mathcal{E}}^{(k)}(\tau,\theta)=\left(\frac{1}{1-\cos\theta}\right)^2\left(\frac{1+\cos\theta}{1-\cos\theta}\right)^{k-1-\frac{1}{4}\frac{D-4}{D-3}}\dot{\mathcal{E}}^{(k)}\left(\bar\tau(\tau,\theta),\frac{\pi}{2}\right)\,,\label{Eq:angular_factorization}
\end{equation}
which proves our proposition.

%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The meaning of perturbation theory}
\label{meaning}
%%%%%%%%%%%%%%%%%%%%%%%%

The perturbative expansion of the metric, Eq.~\eqref{metric_series}, implies an analogous series for the inelasticity's angular distribution $\epsilon(\theta)$ defined in Eq.~\eqref{e1},
\begin{equation}
\epsilon(\theta)=\sum_{N=1}^\infty\epsilon^{(N)}(\theta)\,,
\end{equation}
where
\begin{equation}
\epsilon^{(N)}(\theta)=\sum_{k=1}^{N}\int d\tau\, \dot{\mathcal{E}}^{(k)}(\tau,\theta)\dot{\mathcal{E}}^{(N+1-k)}(\tau,\theta)\,.\label{N_N-k}
\end{equation}

Inserting the result of Eq.~\eqref{Eq:angular_factorization} and changing the integration variable from $\tau$ to $\bar{\tau}$, we conclude that
\begin{equation}
\epsilon^{(N)}(\theta)=\left(\frac{1}{1-\cos\theta}\right)^3 \left(\frac{1+\cos\theta}{1-\cos\theta}\right)^{N-1}\epsilon^{(N)}\left(\frac{\pi}{2}\right)\, . \label{seriesi2}
\end{equation}
%
Thus it suffices to compute the news function on the symmetry plane.

The whole series reads
%
\begin{eqnarray}
\epsilon(\theta)&=&\sum_{N=1}^\infty \epsilon^{(N)}(\theta) =\left(\frac{1}{1-\cos\theta}\right)^3\sum_{N=1}^\infty\left(\frac{1+\cos\theta}{1-\cos\theta}\right)^{N-1}\epsilon^{(N)}\left(\frac{\pi}{2}\right)\,,\\
&\equiv&\sum_{n=0}^\infty\alpha_n(\theta) \epsilon^{(n+1)}\left(\frac{\pi}{2}\right)\,.
\label{series2}
\end{eqnarray}

Observe that each individual $\alpha_n(\theta)$ is regular at $\theta=\pi$, where we saw that perturbation theory should be valid, but does not obey $\alpha_n(\theta)=\alpha_n(\pi-\theta)$ since the transformation to Brinkmann coordinates broke the $\mathbb{Z}_2$ symmetry. However, $\epsilon(\theta)$ should respect that symmetry. In particular, if it has a regular limit at the axis, it can be written as a power series in $\sin^2\theta$,
\begin{equation}
\epsilon(\theta)=\sum_{n=0}^\infty \epsilon_n(\sin\theta)^{2n}\,.\label{angular_series}
\end{equation}

Indeed, writing $\cos\theta=-\sqrt{1-\sin^2\theta}$, we see that near $\theta=\pi$,
\begin{equation}
\alpha_n(\theta)\sim (\sin\theta)^{2n}\,.
\end{equation}

For example, the first three terms are given by
\begin{eqnarray}
\epsilon_0&=&\frac{1}{8}\epsilon^{(1)}\left(\frac{\pi}{2}\right)\,,\label{e0}\\
\epsilon_1&=&\frac{1}{32}\left[3\epsilon^{(1)}\left(\frac{\pi}{2}\right)+\epsilon^{(2)}\left(\frac{\pi}{2}\right)\right]\,,\\
\epsilon_2&=&\frac{1}{128}\left[9\epsilon^{(1)}\left(\frac{\pi}{2}\right)+5\epsilon^{(2)}\left(\frac{\pi}{2}\right)+\epsilon^{(3)}\left(\frac{\pi}{2}\right)\right] \ .
\end{eqnarray}

Thus we conclude that a consistent truncation of the series in Eq.~\eqref{angular_series}, i.e. the extraction of the coefficient $\epsilon_n$, requires knowledge of $\epsilon^{(n+1)}(\tfrac{\pi}{2})$ and hence, from Eq.~\eqref{N_N-k}, of the metric up to $O(n+1)$. This clarifies the meaning of perturbation theory in this problem: it allows for the extraction of successive coefficients $\epsilon_n$, thus amounting to an angular expansion off the collision axis.

It should be stressed that this result is a kinematical consequence of the $CL$ symmetry only: the dynamical (wave) equations have not yet been used (except for the background solution of course).

Finally, the inelasticity is then given by
\begin{eqnarray}
\epsilon&=&\sum_{n=0}^\infty \epsilon_n \int_{-1}^1\frac{d\cos\theta}{2}(\sin\theta)^{2n}\,,\\
&=&\sum_{n=0}^\infty \frac{2^n n!}{(2n+1)!!}\epsilon_n \,,\\
&=&\epsilon_0+\frac{2}{3}\epsilon_1+\ldots\,.\label{eq_second_order_e}
\end{eqnarray}

In the next section we shall obtain simplified expressions for the integrals giving the asymptotic metric functions that contribute to the news function. By working in Fourier space with respect to the retarded time $\tau$, we shall also confirm, explicitly, that the coordinate transformation of Eq.~\eqref{tau_transform} factorises the angular dependence out of the integrals.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Asymptotic integral solution for the metric functions}
\label{asymp_waveforms}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Back in Chapter~\ref{ch:dynamics} we wrote the formal solution for each metric function $F(u,v,\rho)$ in integral form, Eq.~\eqref{sol_3D}. Since we are ultimately interested in the news function $\dot{\mathcal{E}}(\tau,\theta)$, we define the asymptotic waveform $\dot{F}(\tau,\theta)$, obtained from $F(u,v,\rho)$, according to Eq.~\eqref{news2},
\begin{equation}
\dot{F}(\tau,\theta)\equiv\lim_{r\rightarrow\infty} r\rho^{\frac{D-4}{2}}\frac{d}{d\tau}F(u,v,\rho)\,.
\end{equation}

Actually, the Dirac delta in the Green's function is better dealt with in Fourier space, so we define
\begin{equation}
\hat{\dot{F}}(\omega,\theta)\equiv\int d\tau\,\dot{F}(\tau,\theta)e^{-i\omega\tau}\,.
\end{equation}
This is equally useful to compute the inelasticity since, by the Parseval-Plancherel theorem,
\begin{equation}
\int d\tau\, \dot{F}(\tau,\theta)^2=\frac{1}{2\pi}\int d\omega\, |\hat{\dot{F}}(\omega,\theta)|^2\,.
\end{equation}

The next steps are detailed in Appendix~\ref{app:asympWF} due to their tedious and technical nature. 

In short, one needs to take the asymptotic limit and integrate in $\tau$ to obtain the Fourier transform. Dropping primes on integration variables for ease of notation, we get
\begin{equation}
\hat{\dot{F}}(\omega,\theta)=-i^{\frac{D-2}{2}+m}\omega\int_0^\infty d\rho\,\rho^{\frac{D-2}{2}}J_{\frac{D-4}{2}+m}(\omega\rho\sin\theta)\hat{S}\left(\omega\frac{1+\cos\theta}{2},\omega\frac{1-\cos\theta}{2};\rho\right)\,,\label{initial_volume}
\end{equation}
where $J_\nu(z)$ is the $\nu$-th order Bessel function of the first kind and
\begin{equation}
\hat{S}(x,y;\rho)=\frac{1}{2}\int du\int dv\, e^{-iux}e^{-ivy}\, S(u,v,\rho)\,.\label{S_hat}
\end{equation}

Next, one finds it convenient to transform to a new frequency $\Omega$,
\begin{equation}
\omega\rightarrow\Omega\equiv\omega^{D-3}\left(\frac{\sin\theta}{2}\right)^{D-4}\frac{1-\cos\theta}{2}\,,\label{omega_transformation}
\end{equation}
together with a new waveform
\begin{equation}
\hat{\mathcal{F}}(\Omega,\theta)\equiv\sqrt{\omega'(\Omega)}\,\hat{\dot{F}}(\omega(\Omega),\theta)\,,
\end{equation}
such that
\begin{equation}
\int d\omega\, |\hat{\dot{F}}(\omega,\theta)|^2=\int d\Omega\, |\hat{\mathcal{F}}(\Omega,\theta)|^2\,.\label{oO_int}
\end{equation}

Then, using the $CL$ symmetry, namely Eq.~\eqref{def_s}, one shows that, at each order $k$ in perturbation theory,
\begin{equation}
\hat{\mathcal{F}}^{(k)}(\Omega,\theta)=\left(\frac{1}{1-\cos\theta}\right)^{\frac{3}{2}}\left(\frac{1+\cos\theta}{1-\cos\theta}\right)^{k-1}\hat{\mathcal{F}}^{(k)}\left(\Omega,\frac{\pi}{2}\right)\,, \label{angular_factorization}
\end{equation}
where the angular dependence is now completely factored out of the integral, and the (new) Fourier space waveform evaluated at $\theta=\tfrac{\pi}{2}$, which we shall abbreviate to
\begin{equation}
\hat{\mathcal{F}}(\Omega)\equiv\hat{\mathcal{F}}\left(\Omega,\frac{\pi}{2}\right)\,,
\end{equation}
is given by
\begin{equation}
\hat{\mathcal{F}}(\Omega)\equiv -\sqrt{\frac{8}{D-3}}i^{\frac{D-2}{2}+m}\,\Omega^{2k-1}\int_0^\infty dR\,R^{\frac{D-2}{2}}J_{\frac{D-4}{2}+m}(2R)\hat{S}(\Omega^{-1},\Omega;R) \; . \label{Omega_form}
\end{equation}

This formulation in terms of the new frequency $\Omega$ will prove to be useful later on in Chapter~\ref{ch:surface} for the evaluation of surface terms. However, for the time being, we can invert the transformation in Eq.~\eqref{omega_transformation} at $\theta=\tfrac{\pi}{2}$, i.e.
\begin{equation}
\Omega\rightarrow\bar{\omega}\equiv2\,\Omega^{\frac{1}{D-3}}\,,\qquad \hat{\mathcal{F}}(\Omega)\rightarrow\sqrt{\Omega'(\bar{\omega})}\,\hat{\mathcal{F}}\left(\Omega(\bar{\omega})\right)\,.
\end{equation}

The net relationship between $\omega$ and $\bar{\omega}$ is
\begin{equation}
\bar{\omega}=\omega\times(1-\cos\theta)^{\frac{1}{D-3}}(\sin\theta)^{\frac{D-4}{D-3}}\,,
\end{equation}
which is equivalent, in real space, to a transformation of the time coordinate
\begin{equation}
\tau\rightarrow\bar{\tau}(\tau,\theta)=\tau\times(1-\cos\theta)^{-\frac{1}{D-3}}(\sin\theta)^{-\frac{D-4}{D-3}}\,.
\end{equation}
Apart from a $\theta$-dependent shift in $D=4$ (indeed an example of a \emph{supertranslation}~\cite{Coelho:2012sy}) $\bar{\tau}$ is exactly the same as in \eqref{tau_transform}.

In the next chapter we shall specialise this asymptotic solution to the surface case and compute all the terms that contribute to the inelasticity and depend linearly on the initial data. This will allows us to extract the isotropic coefficient $\epsilon_0$.






















